An Algorithm for Computing Lipschitz Inner Functions in Kolmogorov's Superposition Theorem

Kolmogorov famously proved that multivariate continuous functions can be represented as a superposition of a small number of univariate continuous functions, $$ f(x_1,\dots,x_n) = \sum_{q=0}^{2n+1} \chi^q \left( \sum_{p=1}^n \psi^{pq}(x_p) \right).$$ Fridman \cite{fridman} posed the best smoothness bound for the functions $\psi^{pq}$, that such functions can be constructed to be Lipschitz continuous with constant 1. Previous algorithms to describe these inner functions have only been H\"older continuous, such as those proposed by K\"oppen and Braun and Griebel. This is problematic, as pointed out by Griebel, in that non-smooth functions have very high storage/evaluation complexity, and this makes Kolmogorov's representation (KR) impractical using the standard definition of the inner functions. To date, no one has presented a method to compute a Lipschitz continuous inner function. In this paper, we revisit Kolmogorov's theorem along with Fridman's result. We examine a simple Lipschitz function which appear to satisfy the necessary criteria for Kolmogorov's representation, but fails in the limit. We then present a full solution to the problem, including an algorithm that computes such a Lipschitz function.

==> Preamble.tex <==
%% Taken from Dr. Matthew Knepley's CAAM 520 Notes Preamble.tex

\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{amsthm}
\usepackage{mathtools}
\usepackage{bbm}
\usepackage{graphicx}
\usepackage{multirow}
%\usepackage{dtklogos}
\usepackage{wrapfig}
\usepackage{csquotes}
\usepackage{upquote}
\usepackage{eufrak}
\usepackage{mathrsfs}
\usepackage{enumitem}
\usepackage{verbatim}

\usepackage{algorithm}
\usepackage{algorithmicx}
\usepackage[noend]{algpseudocode}

% New definitions
\algnewcommand\algorithmicswitch{\textbf{switch}}
\algnewcommand\algorithmiccase{\textbf{case}}
\algnewcommand\algorithmicassert{\texttt{assert}}
\algnewcommand\Assert[1]{\State \algorithmicassert(#1)}%
% New "environments"
\algdef{SE}[SWITCH]{Switch}{EndSwitch}[1]{\algorithmicswitch\ #1\ \algorithmicdo}{\algorithmicend\ \algorithmicswitch}%
\algdef{SE}[CASE]{Case}{EndCase}[1]{\algorithmiccase\ #1}{\algorithmicend\ \algorithmiccase}%
\algtext*{EndSwitch}%
\algtext*{EndCase}%

% hyperref package should always be loaded as the very last one
% to be sure that it has the last word ...
\usepackage[
    pdftex,
    pdfpagemode={UseOutlines},
    bookmarks, bookmarksopen, bookmarksnumbered={True},
    colorlinks, linkcolor={blue}, citecolor={blue}, urlcolor={blue}
    ]{hyperref}

%% Define a new style for the url package that will use a smaller font.
\makeatletter
\def\url@leostyle{%
  \@ifundefined{selectfont}{\def\UrlFont{\sf}}{\def\UrlFont{\footnotesize\sffamily}}}
\makeatother
%% Now actually use the newly defined style.
\urlstyle{leo}

% TikZ
\usepackage{tikz}
\usepackage{pgflibraryshapes}
\usetikzlibrary{decorations.text}
\usetikzlibrary{decorations.pathreplacing}
\usetikzlibrary{backgrounds}
\usetikzlibrary{calc}
\usetikzlibrary{arrows}
\usetikzlibrary{snakes}
\usetikzlibrary{positioning}
%%\input{figures/tikzColors}
\definecolor{cffffff}{RGB}{255,255,255}
\definecolor{cff00c0}{RGB}{255,0,192}
\definecolor{c0f00ff}{RGB}{15,0,255}
\definecolor{c00ff20}{RGB}{0,255,32}
\definecolor{cfffd00}{RGB}{255,253,0}
\definecolor{c00e0ff}{RGB}{0,224,255}
\usepackage{pgfplots}
\usepackage{pgfplotstable}

% Color macros
\newcommand{\black}{\textcolor{black}}
\newcommand{\blue}{\textcolor{blue}}
\newcommand{\green}{\textcolor{green}}
\newcommand{\red}{\textcolor{red}}
\newcommand{\brown}{\textcolor{brown}}
\newcommand{\cyan}{\textcolor{cyan}}
\newcommand{\magenta}{\textcolor{magenta}}
\newcommand{\yellow}{\textcolor{yellow}}

\usepackage{color}
\definecolor{deepblue}{rgb}{0,0,0.5}
\definecolor{deepred}{rgb}{0.6,0,0}
\definecolor{deepgreen}{rgb}{0,0.5,0}

% Default fixed font does not support bold face
\DeclareFixedFont{\ttb}{T1}{cmtt}{bx}{n}{10} % for bold
\DeclareFixedFont{\ttm}{T1}{cmtt}{m}{n}{10}  % for normal
\DeclareFixedFont{\sttb}{T1}{cmtt}{bx}{n}{8} % for bold
\DeclareFixedFont{\sttm}{T1}{cmtt}{m}{n}{8}  % for normal
% Want a lowercase calligraphic math
\DeclareMathAlphabet{\mathpzc}{OT1}{pzc}{m}{it}
% Font for lstlisting
% \usepackage{courier}

\def\clopt#1{{\tt #1}}
\def\PetscEvent#1{{\tt #1}}

% Vectors
\newcommand{\vF}{\Vec{F}}
\newcommand{\vJ}{\Vec{J}}
\newcommand{\vM}{\Vec{M}}
\newcommand{\vN}{\Vec{N}}
\newcommand{\vU}{\Vec{U}}
\newcommand{\vb}{\Vec{b}}
\newcommand{\vd}{\Vec{d}}
\newcommand{\vf}{\Vec{f}}
\newcommand{\vj}{\Vec{j}}
\newcommand{\vk}{\Vec{k}}
\newcommand{\vn}{\Vec{n}}
\newcommand{\vr}{\Vec{r}}
\newcommand{\vu}{\Vec{u}}
\newcommand{\vv}{\Vec{v}}
\newcommand{\vx}{\Vec{x}}
\newcommand{\vy}{\Vec{y}}
\newcommand{\vz}{\Vec{z}}

\newcommand{\R}{\mathbb{R}}
\newcommand{\C}{\mathbb{C}}
\newcommand{\Q}{\mathbb{Q}}
\newcommand{\Z}{\mathbb{Z}}
\newcommand{\I}{\mathbb{I}}
\newcommand{\N}{\mathbb{N}}
\newcommand{\bb}[1]{\mathbb{#1}}
\newcommand{\curly}[1]{\mathscr{#1}}
\newcommand{\norm}[1]{\left\lVert#1\right\rVert}
\newcommand{\tab}{\hspace{1cm}}

\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\argmax}{arg\,max}

\newtheorem{theorem}{Theorem}[section]
\newtheorem{corollary}{Corollary}[theorem]
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{claim}[theorem]{Claim}
\newtheorem*{remark}{Remark}

\usepackage{listings}

% bash style for highlighting
\newcommand\bashstyle{\lstset{
language=bash,
basicstyle=\scriptsize\ttfamily,
columns=fullflexible
}}

% bash environment
\lstnewenvironment{bash}[1][]
{
\bashstyle
\lstset{#1}
}
{}

% bash for inline
\newcommand\bashinline[1]{{\bashstyle\lstinline!#1!}}


% make style for highlighting
\newcommand\makestyle{\lstset{
language=make,
basicstyle=\scriptsize\ttfamily,
columns=fullflexible
}}

% make environment
\lstnewenvironment{make}[1][]
{
\makestyle
\lstset{#1}
}
{}

% make for inline
\newcommand\makeinline[1]{{\makestyle\lstinline!#1!}}

% Python style for highlighting
\newcommand\pythonstyle{\lstset{
language=Python,
basicstyle=\sttm,
otherkeywords={self},             % Add keywords here
keywordstyle=\sttb\color{deepblue},
emph={MyClass,__init__},          % Custom highlighting
emphstyle=\sttb\color{deepred},    % Custom highlighting style
commentstyle=\sttm\color{deepgreen},
frame=tb,                         % Any extra options here
showstringspaces=false,           %
columns=fullflexible              % Necessary for proper cut/paste
}}

% Python style for inline highlighting
\newcommand\pythoninlinestyle{\lstset{
language=Python,
basicstyle=\ttm,
otherkeywords={self},             % Add keywords here
keywordstyle=\ttb\color{deepblue},
emph={MyClass,__init__},          % Custom highlighting
emphstyle=\ttb\color{deepred},    % Custom highlighting style
commentstyle=\ttm\color{deepgreen},
frame=tb,                         % Any extra options here
showstringspaces=false,           %
columns=fullflexible              % Necessary for proper cut/paste
}}

% Python environment
\lstnewenvironment{python}[1][]
{
\pythonstyle
\lstset{#1}
}
{}

% Python for external files
\newcommand\pythonexternal[2][]{{
\pythonstyle
\lstinputlisting[#1]{#2}}}

% Python for inline
\newcommand\pythoninline[1]{{\pythoninlinestyle\lstinline!#1!}}

% C style for highlighting
\newcommand\cstyle{\lstset{
language=C,
basicstyle=\sttm,
otherkeywords={MPI_Comm,TS,SNES,KSP,PC,DM,Mat,Vec,VecScatter,IS,PetscSF,PetscSection,PetscObject,PetscInt,PetscScalar,PetscReal,PetscBool,InsertMode,PetscErrorCode}, % Add keywords here
keywordstyle=\sttb\color{deepblue},
emph={PETSC_COMM_WORLD,PETSC_NULL,SNES_NGMRES_RESTART_PERIODIC},          % Custom highlighting
emphstyle=\sttb\color{deepred},    % Custom highlighting style
commentstyle=\sttm\color{brown},
stringstyle=\sttm\color{deepgreen},
frame=tb,                         % Any extra options here
showstringspaces=false,           %
columns=fullflexible              % Necessary for proper cut/paste
}}

\newcommand\cinlinestyle{\lstset{
language=C,
basicstyle=\ttm,
otherkeywords={MPI_Comm,TS,SNES,KSP,PC,DM,Mat,Vec,VecScatter,IS,PetscSF,PetscSection,PetscObject,PetscInt,PetscScalar,PetscReal,PetscBool,InsertMode,PetscErrorCode}, % Add keywords here
keywordstyle=\ttb\color{deepblue},
emph={PETSC_COMM_WORLD,NULL,SNES_NGMRES_RESTART_PERIODIC},          % Custom highlighting
emphstyle=\ttb\color{deepred},    % Custom highlighting style
commentstyle=\ttm\color{brown},
stringstyle=\ttm\color{deepgreen},
frame=tb,                         % Any extra options here
showstringspaces=false,           %
columns=fullflexible              % Necessary for proper cut/paste
}}

% C environment
\lstnewenvironment{cprog}[1][]
{
\cstyle
\lstset{#1}
}
{}

% C for external files
\newcommand\cexternal[2][]{{
\cstyle
\lstinputlisting[#1]{#2}}}

% C for inline
\newcommand\cinline[1]{{\cinlinestyle\lstinline!#1!}}

